Incorporating Different Verbal Cues to Improve Text-Based Computer-Delivered Health Messaging

The ubiquity of smartphones has led to an increase in on demand healthcare being supplied. For example, people can share their illness-related experiences with others similar to themselves, and healthcare experts can offer advice for better treatment and care for remediable, terminal and mental illnesses. As well as this human-to-human communication, there has been an increased use of human-to-computer digital health messaging, such as chatbots. These can prove advantageous as they offer synchronous and anonymous feedback without the need for a human conversational partner. However, there are many subtleties involved in human conversation that a computer agent may not properly exhibit. For example, there are various conversational styles, etiquettes, politeness strategies or empathic responses that need to be chosen appropriately for the conversation. Encouragingly, computers are social actors (CASA) posits that people apply the same social norms to computers as they would do to people. On from this, previous studies have focused on applying conversational strategies to computer agents to make them embody more favourable human characteristics. However, if a computer agent fails in this regard it can lead to negative reactions from users. Therefore, in this dissertation we describe a series of studies we carried out to lead to more effective human-to-computer digital health messaging. In our first study, we use the crowd [...] Our second study investigates the effect of a health chatbot's conversational style [...] In our final study, we investigate the format used by a chatbot when [...] In summary, we have researched how to create more effective digital health interventions starting from generating health messages, to choosing an appropriate formality of messaging, and finally to formatting messages which reference a user's previous utterances.

==> 1-OLD-Chapter-Introduction.tex <==
\chapter{Introduction}

% This is one of the most important components of the report. It should begin with a clear statement of what the project is about so that the nature and scope of the project can be understood by the reader. It should summarise everything you set out to achieve, provide a clear summary of the project's background and relevance to other work, and give pointers to the remaining sections of the report that contain the bulk of the technical material. 

%This dissertation investigates how people can be motivated to inherently change their physical activity behavior through theory-based and tailored interventions in the form of motivational text messages delivered by technology. Section 1.1 explains what reasoning has lead to choosing theory-based and tailored interventions to motivate people to change their physical activity behavior. Section 1.2 presents the research questions that are addressed. Section 1.3 explains the approach taken to answer these research questions. Lastly, section 1.4 provides an outline for the following chapters.

This dissertation investigates the use of technology for text-based messaging to assist users in developing healthy habits, and describes several of our studies that answer related research questions.
%, and we will describe several studies we used to investigate the generation and use of text-based messaging.
%As a high-level goal we want to produce messaging that is more efficacious and ``human-like''.
%We will describe several studies we have undertaken to produce more human-like messages. 
%This could be in the generation of health content, and user perception of a computer's communication.
In this introduction chapter, Section \ref{ch1:motivation} describes the motivation behind our work, and the context behind each of our studies.
Section 1.2 lays out our research questions, and explains the methods used to answer them.
Finally, Section \ref{ch1:outline} outlines the rest of the chapters of this report.
%In section \ref{ch1:motivation} we will describe the overall motivation of our studies, and how our research questions contribute to solving outstanding issues. Finally in Section \ref{ch1:outline} outlines the rest of the chapters of this report.





Beyond this introduction, the dissertation describes work from three sets of studies.
%First, we investigated how to generate \textit{diverse} motivational messages. 
In our first study, we developed and evaluated a system to scalably and automatically direct the crowd to generate diverse health messages.
%In our second set of studies, we investigated the conversational style of a disembodied chatbot, and its effect on the quality of a user's information sharing. 
In our second study, we investigated the effect of a health chatbot's conversational style in a series of user studies, and found that a formal conversational style may lead to higher quality user responses compared to a casual style.
%In our final study, we will investigate when it is best for a health chatbot to seek expert human assistance.
%\textcolor{thesis}{In our final study, we will investigate the effect of a chatbot referencing previous user utterances on a user's response quality.}
In our final study, we varied the format of how a health chatbot references a user's utterances from a previous chatting session to investigate its effects on a user's positive perceptions, and privacy concerns.
%In our final study, we will investigate when it is best for a health chatbot to seek expert human assistance, and we aim to generate design guidelines for chatbot mediated patient-doctor communication.


\section{Motivation}
\label{ch1:motivation}


There are many health guidelines we are told to follow such as getting enough exercise \cite{fiuza2013exercise}, eating a balanced and healthy diet \cite{healthhub}, %https://www.healthhub.sg/programmes/191/nutrition-hub/eat-more
getting enough sleep \cite{ohayon2017national}, or completing medication prescriptions. 
Although following such guidelines could lower our risk of chronic illnesses, we may not always succeed in doing so without social support \cite{brown1986social,cohen2007social,duncan1993social}.

%Social support can help people perform more healthy behaviours \cite{brown1986social,cohen2007social}, in part by improving a person's self-efficacy \cite{duncan1993social}.

Historically, this support could be in the form of friends, family members or health professionals. However, this support may not always be available to people when they need it most. People may be too busy to support others, and health professionals may not be accessible to everyone due to cost or scheduling issues. 
%Review of chatbots for weight-loss \cite{chew2022use}.
A potential alternative form of social support comes from the use of messaging technology \cite{adams2014staccato,ta2020user,benavente2023replacing}.

Health messaging technology is something many people have already adopted into their daily lives \cite{wasil2022there,tudor2020conversational,chew2022use}.
It ranges from one-off nudging such as smartphone applications that send notifications to remind someone to exercise \cite{rabbi2015mybehavior}, to longer conversational interventions such as chatbots that discuss someone's cancer diagnosis \cite{chaix2019chatbots}.
%Additionally, health technology is becoming accessible to more people and as of 2020 nearly 50\% of the world population owns a smartphone \cite{odea_2021}.
Furthermore, as a computer does not need to ``sleep'' messages can be sent synchronously at any time, unlike people who may not always be available.
Additionally, the technology that makes this possible is becoming accessible to more people, and as of 2020 nearly 50\% of the world population owns a smartphone \cite{odea_2021}.
This gives the option for low-cost and highly accessible support for people with their health needs, as the technology is scalable provided that infrastructure (such as reliable Internet or phone service) exists.


Health technology, such as chatbots, have already seen some acceptance from both consumers \cite{nadarzynski2019acceptability} and medical professionals \cite{palanica2019physicians}.
Physicians described their support of health chatbots for providing information and scheduling appointments (but also professed a scepticism in a chatbot's ability to diagnose health problems) \cite{palanica2019physicians}.
Consumers have described how they value the anonymity and convenience of health chatbots, and that they may be willing to share symptoms with chatbots \cite{nadarzynski2019acceptability}.
However, both physicians and consumers raised lack of empathy and inability to understand human emotions as potential barriers to engagement with health chatbots.

These concerns lead us to a potential impasse. Namely, the question of ``\textit{How} should technology communicate with us?''.
%How should messages for technology be written?
We want technology which people perceive as understanding their emotions and that responds empathetically. 
However, we don't want technology which enters the uncanny valley \cite{ho2008human,wozniak2021creepy} where communication is seen as \textit{almost} human-like, but something is not quite right.
Equally we don't want technology which responds in a way seen as inappropriate to the situation \cite{cox2022does,chaves2019s}.
%If we want health technology to be adopted, how can we make it feel more human-like, without entering into the uncanny valley of communication?
For example, users may find it more appropriate if a chatbot uses a more formal conversational style when discussing their personal health \cite{cox2022does}.
%For example, would we expect a chatbot which administers health advice to use a highly casual tone, or would we prefer a more formal style?

Improving the humanness of computer communications has already been the focus of much research \cite{lin_caire_2020,xiao2020tell,liu2018should,volkel2022user,brown_politeness_1987}.
One paradigm that has led this drive is the ``Computers are social actors'' (CASA) paradigm \cite{nass1994computers}. CASA states that people apply the same social heuristics to computers as they do to humans. For example, people may carry forward their own existing gender biases when interacting with an agent \cite{mcdonnell2019chatbots}, or may expect the same politeness conventions to be upheld \cite{brown_politeness_1987,chaves2021should}.
The CASA paradigm has thereby encouraged people to develop computers which communicate using favourable human traits (such as a tone-aware customer care chatbot \cite{hu2018touch}), or that exploit human biases (such as a chatbot which mirrors a user's race \cite{liao_racial_2020}).
% Do I need a section here which briefly describes previous work that people have done?
% I.e., "This study made a tone-aware chatbot for customer service" etc.
% Do I need to better state why this is difficult, and why we are still investigating it? If it's been the "focus of much research" then why do people still care?
%Furthermore, chatbots have been found to benefit from various human-like qualities such as empathy \cite{lin_caire_2020}, listening \cite{xiao2019tell}, differing conversational styles and personas \cite{liu2018should,volkel2022user}, and adopting favourable politeness strategies \cite{brown_politeness_1987}.


This desire to create more human-like and appropriate computer communication is the main motivation behind our studies. We want to create computer health messaging which is perceived more positively by people, so as to better help them meet their health needs.
%Previous work have focused on the use of technology to improve people's health. This could be to tackle the rise in chronic diseases due to diet or sedentary lifestyles, mental health problems, medication non-adherence, or insomnia \cite{hekler2013mind}.
%Wei Tsang - Mon 24th May - Chatbots, intervention messaging (apps that people use everyday?). Health messaging. How deliver. through notifications, adverts, chatbots (so interactive). Why interactive messaging important. Human-like (CASA). Vik for cancer, mental health chatbot. 
We focus on computer messaging both at the conception stage (with the generation and curation of efficacious messages), and the end-user stage with empirical studies to investigate what makes health messaging more effective.
We will describe the literature related to these processes in the related work chapter that follows, and outline how our studies attempt to further the knowledge of each section.
%We are interested in computer health messaging as an end to end process of (1) generating and curating content; (2) selecting content for interactions; and (3) determining the most appropriate context for an agent to seek human interventions. We will describe the literature related to these processes in the related work chapter that follows, and outline how our studies attempt to further the knowledge of each section.
%(see \textbf{Figure \ref{fig:Background-diagram}} for a high level view of how our three studies fit together).


Our first studies in \textbf{Chapter 3} draw on the crowd to generate diverse health messaging, which can be used as interventions or to train chatbots. 
For this, we developed and evaluated a method to scalably and automatically generate more diverse health messages by using embedding distances to send crowd-workers collectively diverse phrases to inspire their ideation.
Our studies in \textbf{Chapter 4} draw a connection between health chatbots and their users. 
More specifically, we investigated the effect of a health chatbot's conversational style, and found that a formal conversational style may lead to higher quality user responses. 
%Finally, our study in \textbf{Chapter 5} will make a connection between chatbots, users, and human experts.
%We will investigate under what circumstances a health chatbot should seek expert human intervention.
Finally, our study in \textbf{Chapter 5} investigated the effect of varying how a chatbot refers to user utterances from a previous chatting session, and we found that, while people think more positively of chatbots that explicitly reference their previous utterances, they also find them more privacy violating.
%\textcolor{thesis}{Finally, our study in \textbf{Chapter 5} will again investigate how to improve user response quality to a health chatbot. In this study, we will investigate the effect of a chatbot referencing previous user utterances both in its occurrence, and in the format of referencing.}

Now that you've seen an overview of the studies in the dissertation, we will describe our research questions.


\section{Research Questions}


This dissertation aims to improve the effectiveness of text-based computer-delivered health messaging.
We believe that messaging can be improved: (1) in the way it is generated; (2) by adopting an appropriate style for health communication; and (3) by altering the presence and format of a chatbot's references to previous user utterances.
The high-level research question of this dissertation is therefore:

%Wei Tsang: Why important to be human-like?
\begin{displayquote}
    \textbf{How can we make text-based computer-delivered health messaging more effective?}
\end{displayquote}

Below we will outline our three studies in more detail, and their corresponding high-level research questions.

\subsection{Generating Diverse Health Content}

Our first study investigates how health messaging can be generated. One method to generate large amounts of health content is to use collections of people hereby referred to as ``the crowd'' \cite{de2016crowd}.
Previous work has studied how to use the crowd to generate health content such as motivational messages \cite{de2016crowd}, exercise plans \cite{agapie2016plansourcing}, and solutions to back pain \cite{hosio2018crowdsourcing}. 
Using the crowd is low cost (compared to using experts), and can generate personable and relatable content by drawing on people's personal experiences \cite{coley2013crowdsourced}.
The ability to produce large amounts of health content is particularly useful for interventional messaging or chatbots, where a large amount of messages are needed both to avoid user boredom in repeated interventions \cite{kocielnik2017send}, and in order to train algorithms for chatbot systems.

%The ability to produce large amounts of health content is particularly useful for both interventional messaging or chatbots.
%This repeated content causes additional issues with regards to health messaging.
%As behaviour change is typically a long-term process, messaging needs to be repeated over long period of time \cite{consolvo2014designing}. However, seeing the same or similar messages repeatedly can lead to boredom, annoyance, content blindness or even avoidance, resulting in poor adherence and dropouts \cite{cacioppo1979effects,strecher2005randomized}. 

% Why important? Why challenging? (why can't undergrad do?). Why is it interesting?
%Wei Tsang: How do this? Why low cost? What are challenges? Show difficulties and challenges.

However, the crowd may produce similar or identical ideas, which leads to redundancy and wasted human effort \cite{bayus2013crowdsourcing,bjelland2008inside}.
Previous work within crowdsourcing and creativity have shown example ideas to the crowd to help them generate diverse ideas \cite{siangliulue2016ideahound,huang2017bluesky}, but these systems often rely on manual human effort to run. We want to use the crowd to generate \textit{diverse} health messages, while also using a \textit{scalable} and more \textit{automatic} system.
This leads us to our first research question:

\vspace{5mm}
\textit{\textbf{RQ1:} How can we use the crowd to automatically and scalably generate diverse health messaging?}
\vspace{5mm}

To help answer this we developed \textit{Directed Diversity}  \cite{cox2021diverse}, a method which harnesses embedding distances to scalably and automatically allocate diverse example ideas to crowd-workers.
By giving diverse examples to workers, we generate a \textit{collectively diverse} corpus of messages.
In our user studies we showed users short phrases related to physical exercise (e.g., ``hard workout may feel'') to inspire workers to write motivational messages to encourage exercise.
To automate our process, we used existing online health content to generate the examples shown to workers, and developed an algorithm to select semantically diverse examples to show to workers.
%In a series of user studies we used the crowd to generate motivational messages to encourage physical activity.
%Motivational messages increase the odds of behaviour change when used appropriately. Such messages have been used in several areas, such as to ensure medication adherence \cite{kreps2011development}, to assist smoking cessation \cite{ghorai2014mhealth}, to reduce alcohol consumption \cite{kristan2015using}, and to encourage physical activity \cite{hekler2013mind,milne2002combining}.
To measure the efficacy of our crowd-generated messages, we asked people to hypothetically answer how they themselves would find the message if it was a notification on their phone.
We also used human evaluations and objective measures to evaluate the diversity of messages.
It was found that our method helped the crowd generate diverse content when compared to both randomly selected examples and no examples, while still generating efficacious motivational messages. This is described in detail in Chapter \ref{ch:DirectedDiversity}.



%Hence, researchers have called for the need to diversify messaging \cite{kocielnik2017send,pechmann1988advertising} and attempted to offer practical methods to create diversity, such as Kocielnik and Hsieh's \cite{kocielnik2017send} use of strategies based on cognitive space.
%Kocielnik and Hsieh \cite{kocielnik2017send} produced diverse messages to encourage physical exercise based on target-diverse (cognitively close to target action) and self-diverse (cognitively close to message recipient) messages. They found cognitively diverse messages, maintained the same quality and meaning, but did not encounter the same negative effects of repeated exposure.
%De Vries et al. crowdsourced motivational messages to encourage exercise based on the stages of change \cite{de2016crowd}. To better control crowdsourcing of messages for each stage of change, they used scenarios to elicit responses from participants.
%Additionally within creativity literature methods have been proposed which give crowd-workers examples to help generate diverse content \cite{siangliulue2016ideahound,huang2017bluesky,girotto2019crowdmuse}.
%However these methods are not fully-automated and rely on manual effort to label idea categories, or are restricted to a discrete number of idea categories.

\subsection{Choosing an appropriate conversational style for a health chatbot}

In our second study, we investigated the effect of a health chatbot's conversational style on a user's quality of information disclosure.
%Disembodied (text-based without an avatar) chatbots have been used in healthcare such as for cancer information giving \cite{chaix2019chatbots}, improving mental health \cite{liao2020personalized,park_designing_2019}, and for encouraging physical exercise \cite{kocielnik_reflection_2018}.
In order to help people improve their health, chatbots need to be given enough information. However, people may be unwilling to disclose their information if a chatbot is perceived negatively \cite{palanica2019physicians}.
Previous work has investigated the effect of conversational style on quality of multiple-choice survey responses, both with a standard survey and with a survey chatbot \cite{kim_comparing_2019}.
However, we are interested in the effect of conversational style on the quality of disclosure to a health chatbot, in terms of likelihood to disclose and quality of user utterances.
This led us to our second research question of:

\vspace{5mm}
%What is the effect of a chatbot's language formality on a user's self-disclosure?
\textit{\textbf{RQ2:} How does the conversational style (i.e., language formality) of a health chatbot affect the quality of a user's self-disclosure?}
\vspace{5mm}

On from this, we investigated the effect of a health chatbot's conversational style on the quality of response from users \cite{cox2022does}.
We conducted two user studies to investigate the impact formal and casual conversational styles on human perceptions (such as likelihood to disclose, and perceptions of the chatbot) and the quality of responses given to the chatbot. 
In our study users perceived a formal conversational style to be more appropriate and competent, and a formal conversational style was found to produce more informative user utterances. We describe this study in detail in Chapter 4.

%\subsection{Investigating the appropriate time for a health chatbot to seek assistance from a health expert}

\subsection{Changing the format of a health chatbot's references to a user's previous utterances}

%While chatbots can be used to assist people with their health needs, the input of human experts may still be necessary in certain situations.
%For example, a chatbot may not have sufficient domain knowledge (or confidence) to answer certain health questions; some topics may be deemed too sensitive for a chatbot to answer (either in terms of privacy or potential affects on health); or a user may desire additional emotional support from a human rather than a chatbot.
%For this reason, a chatbot should be aware of when it needs to alert a human expert for assistance. This leads us to our third research question of:


Health interviewers have been found to be effective both by adopting higher levels of social presence \cite{tsaihuman,xiao2020tell} (such as paraphrasing a user's utterances) or by adopting lower levels of social presence \cite{schuetzler2018influence,chen2021you,ng2020simulating} (such as by providing high-level references to user utterances).
These two conflicting schools of thought lead us to investigate the effect of varying levels of social presence (via the ability of a chatbot remembering previous user utterances).
This leads us to our third research question of:

\vspace{5mm}
%\textit{RQ3: When should a health chatbot seek assistance from a human expert?}
\textit{\textbf{RQ3:} How does the format used when a chatbot references a user's utterances from previous chatting sessions impact a user's perception of a chatbot and why?}
%\textit{RQ3: How does the presence and format of a chatbot's references to previous user utterances affect user perceptions and privacy concerns?}
\vspace{5mm}

As a result of this, we conducted a between subjects longitudinal study where we varied the format a chatbot would use when referencing user utterances from previous chatting sessions.
We found that people find a format which references their past utterances explicitly makes the chatbot seem more intelligent and engaging to users, but also raises privacy concerns. We then conducted semi-structured interviews to further investigate \textit{why} people viewed the referencing formats differently.
This study is described in Chapter 5.

%\textcolor{thesis}{To answer this, we will carry out a longitudinal between-subjects experiment where participants will talk to a chatbot about their dental flossing. The chatbot will vary in whether it remembers previous user utterances and in the format it uses to reference previous user utterances back to the user. This study is described in Chapter 5.}
%To answer this, we aim to investigate the use of a chatbot to facilitate conversations between doctors and patients.
%Our study will be based on a ``group-chat'' of a doctor, a patient and a chatbot.
%We will investigate the most appropriate contexts for a chatbot to seek assistance from a human expert. This study is described in Chapter 5.

\section{Thesis Outline}
\label{ch1:outline}

In this thesis, I will outline background literature, as well as the three sets of studies that we have completed. 
The structure of this report is outlined below:

\subsubsection{Chapter \ref{ch:background}: Background Research and Related Work}

This chapter investigates the topics related to the project and outlines any relevant research. 
In our related work chapter, we contextualise our 3 studies by providing a background overview of health communication technology.
As we are interested in text-based health messaging, we first start by giving an overview of health message generation and curation.
We then describe previous work that has attempted to improve health messaging technology, such as by adopting conversational style.

We focus on health communication technology, and more specifically are interested text based communication such as nudges or conversations to encourage healthy behaviours.

\subsubsection{Chapter 3: Generating Diverse Prompts}
In order to maintain user interest, and be more efficacious across different cohorts a diverse range of health messages is needed. Therefore we conducted a study to crowd-source diverse health prompts by harnessing the power of embedding distances. We found that our crowd-sourcing method led to more diverse and informative messages compared to two baseline methods. 
This study is published as:

\bibentry{cox2021diverse}


\subsubsection{Chapter 4: Choosing health chatbot conversational style}
The conversational style of a health chatbot impacts efficacy and user perceptions. 
Therefore we carried out a study to investigate the effectiveness of both formal and casual conversational styles. 
In our study users perceived a formal conversational style to be more appropriate and competent, and a formal conversational style was found to produce more informative user responses.
This study is published as:

\bibentry{cox2022does}

\subsubsection{Chapter 5: How should a health chatbot remember and reference previous user utterances?}

This upcoming study will investigate the effect of a health chatbot remembering and referencing previous user utterances on the quality of user utterances.
Particularly we will vary the presence and format and references to previous user utterances.
This study is being revised before submission to a relevant publication.

%\subsubsection{Chapter 5: A patient, a doctor and a chatbot enter a group-chat...}

%This upcoming study will investigate the use of a chatbot to facilitate communication between a doctor and a patient.
%Within our context, a chatbot could be used to communicate with a patient to respond promptly while freeing up a doctor's time.
%However, it is not always clear when a doctor should intervene, and under what context a chatbot should prompt a doctor for intervention into a conversation.
%We will examine the conversational content deemed appropriate for a chatbot in such a scenario, and the opportune moment for a chatbot to communicate with a doctor (such as to request further information or to alleviate a patient's anxieties).

%This upcoming study will investigate the optimal way to enlist a doctor (or expert) for help when a patient needs it. It will investigate the optimal time to interrupt a doctor, the most appropriate amount of information to exchange, and the most appropriate form of information summarisation to deploy.
%We aim to publish this study in CSCW.

%It will be a comparative study between different interruption times (no interruptions/help, scheduled interruption, user requested interruption), summarisation method (similar to those in "Bot in the Bunch"?), and the amount of information exchanged.

%We will measure the effect on both patient and doctor perceptions.

%\subsubsection{Chapter 6: BarrierBot}
%In one of our upcoming studies we will develop a chatbot to help user's identify their barriers to healthy behaviour (in this case dental flossing). 
%Our system (``BarrierBot'') will deliver appropriate and empathic utterances to users.
%We will test the efficacy of the chatbot in a longitudinal study against a baseline.


%\subsubsection{Chapter 7: A review of chatbot conversational styles of existing health chatbots}
%This study will analyse the conversational style deployed by existing health chatbots.

%\subsubsection{Chapter 7: A heuristic health bot}
%People use heuristics to help them make decisions. For different chatbot tasks (information giving, information taking, rapport growing,...) which heuristics are most recommended to harness and why?

\subsubsection{Chapter 6: Conclusion}
This chapter reflects on the current and expected achievements of the project.

\vspace{10mm}

%It is also worth noting that (unless otherwise stated) all diagrams are produced using the online diagram software \url{www.gliffy.com}.
